Analytically-Driven Resource Management for Cloud-Native Microservices

Resource management for cloud-native microservices has attracted a lot of recent attention. Previous work has shown that machine learning (ML)-driven approaches outperform traditional techniques, such as autoscaling, in terms of both SLA maintenance and resource efficiency. However, ML-driven approaches also face challenges including lengthy data collection processes and limited scalability. We present Ursa, a lightweight resource management system for cloud-native microservices that addresses these challenges. Ursa uses an analytical model that decomposes the end-to-end SLA into per-service SLA, and maps per-service SLA to individual resource allocations per microservice tier. To speed up the exploration process and avoid prolonged SLA violations, Ursa explores each microservice individually, and swiftly stops exploration if latency exceeds its SLA. We evaluate Ursa on a set of representative and end-to-end microservice topologies, including a social network, media service and video processing pipeline, each consisting of multiple classes and priorities of requests with different SLAs, and compare it against two representative ML-driven systems, Sinan and Firm. Compared to these ML-driven approaches, Ursa provides significant advantages: It shortens the data collection process by more than 128x, and its control plane is 43x faster than ML-driven approaches. At the same time, Ursa does not sacrifice resource efficiency or SLAs. During online deployment, Ursa reduces the SLA violation rate by 9.0% up to 49.9%, and reduces CPU allocation by up to 86.2% compared to ML-driven approaches.

==> benchmark_full.tex <==
\section{Benchmarks}
\label{sec:benchmark}

%\sameh{Shall we call it benchmarks and implementation? how many lines of code in each app? How about Ursa?}
%\yanqi{I think it might be clearer to talk about impl of Ursa itself in the previous Ursa design \& impl section?}

Conventional microservice benchmarks~\cite{gan2019open, sriraman2018mu, zhou2018fault} face several limitations. 
First, conventional benchmarks use RPC as the only method for inter-service communication, whereas MQs also common in practice~\cite{luo2021characterizing}. 
Second, the business logic of conventional benchmark involves only lightweight text processing, whereas a modern microservice can handle different user request classes performing tasks, such as image processing and ML workloads~\cite{shahrad2020serverless, mahgoub2022orion, romero2021faast}, and even different request priorities, making resource management more challenging.
To address these limitations, we implement three benchmark applications using Dapr~\cite{dapr}, a popular microservice framework developed and used by major cloud providers, as described below. 
For all the applications, we implement the business logic in Golang and Python, and use gRPC~\cite{gRPC} as RPC, Redis streams~\cite{redis-streams} as message queues and Redis~\cite{redis} as data stores. 

% \begin{figure}[t]
% \centering
% \includegraphics[width=.95\linewidth]{benchmark_social_network.pdf}
% % \vspace{-0.16in}
% \caption{Social network.}
% \label{fig:socialnet}
% % \vspace{-0.16in}
% \end{figure}

\myparagraph{Social network} The social network application is inspired by Deathstar benchmark~\cite{gan2019open} and its topology is shown in Figure~\ref{fig:socialnet}. 
\sameh{Bad reviewer: Authors have changed the benchmark to avoid apples to apples comparison. I really want to see the Deathstart results.}
The application uses both RPC and message queue for inter-service communication, marked by black and red arrows in Figure~\ref{fig:socialnet}, respectively. 
% Compared to Deathstar that supports only uploading text posts and reading timelines, 
In addition to uploading text posts and reading timelines, 
social network implements several new features, including support for post with images, upvote, comment, friend recommendation, translation, sentiment analysis of texts and object detection of images. Translation, sentiment analysis and object detection are implemented with machine learning models from Hugging Face~\cite{huggingface}.
Different request paths have diverse latency, ranging from tens of milliseconds for comment, to over a hundred milliseconds for image upload, to hundreds or thousands of milliseconds for machine learning tasks. Different request paths also share services. For example, both comment and image upload goes through the Frontend service.

\begin{figure}[t]
\centering
\includegraphics[width=.95\linewidth]{benchmark_video_sharing.pdf}
% \vspace{-0.16in}
\caption{Video sharing.}
\label{fig:video-sharing}
\vspace{-0.16in}
\end{figure}

\myparagraph{Media service} The video sharing application is also inspired by Deathstar, with the topology shown in Figure~\ref{fig:video-sharing}. Similar to social network, both RPC and message queue are used in the application. In addition to reviewing and rating videos, video sharing allows users to upload and download actual video, and implements video-processing tasks such as scaling to different resolutions and generating thumbnail images via FFmpeg~\cite{ffmpeg}. The latency of requests ranges from tens of milliseconds for rate and review, to a tens of seconds for video scaling. Services also handle different types of request with different latency. For example, in the Frontend service, it takes tens of milliseconds to process a rate request, and hundreds of milliseconds to extract video metadata via FFmpeg.

\myparagraph{Video processing pipeline} Video processing pipeline consists of three stages, the first stage extracts video metadata, the second stage takes snapshots from the video at fixed intervals, and the third stage performs face recognition on the video snapshots. The first two stages are implemented with FFmpeg and the third stage is implemented with OpenCV~\cite{opencv}.
Each stage has a worker thread pool, and  requests are first put into a queue and then processed by an idle thread.
More importantly, the application handles requests with two different priorities. High-priority requests are always processed immediately when there are available threads, while low-priority requests are processed only when there are no high-priority request waiting in the queue. 

\begin{figure}[t]
\centering
\includegraphics[width=.95\linewidth]{benchmark_video_pipeline.pdf}
% \vspace{-0.16in}
\caption{Video processing pipeline.}
\label{fig:video-pipe}
\vspace{-0.2in}
\end{figure}

\begin{table}[h]
\centering
\begin{small}
\begin{tabular}{ll}
Request type        & $99^{th}$ latency (ms) \\ \midrule
post/comment/upvote & $75$   \\
read-timeline       & $250$   \\
update-timeline     & $500$   \\
upload-image        & $200$   \\
download-image      & $75$   \\
sentiment-analysis  & $500$   \\
object-detect       & $10000$     \\ \bottomrule  
\end{tabular}
\end{small}
\caption{SLAs of social network application.}
\label{tab:sla_social}
\vspace{-0.35in}
\end{table}

\begin{table}[h]
\centering
\begin{small}
\begin{tabular}{ll}
Request type        &  $99^{th}$ latency (ms) \\ \midrule
upload-video        & $2000$   \\
download-video      & $1500$   \\
get-info            & $250$   \\
rate-video          & $400$   \\
scale-video         & $40000$   \\
generate-thumbnail  & $2000$     \\ \bottomrule  
\end{tabular}
\end{small}
\caption{SLAs of video sharing application.}
\label{tab:sla_video_share}
\vspace{-0.24in}
\end{table}

\begin{table}[h]
\centering
\begin{small}
\begin{tabular}{lll}
Request type        & Percentile & Latency (ms) \\ \midrule
high-priority       & $99^{th}$         & $20000$   \\
low-priority        & $50^{th}$         & $4000$   \\ \bottomrule  
\end{tabular}
\end{small}
\caption{SLAs of video processing pipeline.}
\label{tab:sla_video_pipe}
\vspace{-0.35in}
\end{table}

